RotNet: Fast and Scalable Estimation of Stellar Rotation Periods Using Convolutional Neural Networks

Magnetic activity in stars manifests as dark spots on their surfaces that modulate the brightness observed by telescopes. These light curves contain important information on stellar rotation. However, the accurate estimation of rotation periods is computationally expensive due to scarce ground truth information, noisy data, and large parameter spaces that lead to degenerate solutions. We harness the power of deep learning and successfully apply Convolutional Neural Networks to regress stellar rotation periods from Kepler light curves. Geometry-preserving time-series to image transformations of the light curves serve as inputs to a ResNet-18 based architecture which is trained through transfer learning. The McQuillan catalog of published rotation periods is used as ansatz to groundtruth. We benchmark the performance of our method against a random forest regressor, a 1D CNN, and the Auto-Correlation Function (ACF) - the current standard to estimate rotation periods. Despite limiting our input to fewer data points (1k), our model yields more accurate results and runs 350 times faster than ACF runs on the same number of data points and 10,000 times faster than ACF runs on 65k data points. With only minimal feature engineering our approach has impressive accuracy, motivating the application of deep learning to regress stellar parameters on an even larger scale

==> sections/2_data.tex <==
% \begin{figure}[h!]
% \small
% \begin{center}
% \includegraphics[width=140mm]{figures/tsimage.jpg}
% \caption{Some representative Light Curves and their corresponding Image Transformations. The \textbf{top row} shows a light curve with a fast rotation period and the \textbf{bottom row} shows a light curve with a slow rotation period along with their respective image transformations } % used as stopping criterion with the 
% \label{fig:ts2img}
% \end{center}
% \end{figure}

% \begin{figure}[h!]
% \small
% \begin{center}
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{cccc}
% Light Curve & GAF & MTF & RP \\[0mm]
% \includegraphics[width=5.0cm,height=3.0cm]{figures/ts2img/fig2_fast_lc.pdf} &
% \includegraphics[width=3.5cm,height=3.5cm]{figures/ts2img/fig2_fast_gaf.pdf} &
% \includegraphics[width=3.5cm,height=3.5cm]{figures/ts2img/fig2_fast_mtf.pdf} &
% \includegraphics[width=3.5cm,height=3.5cm]{figures/ts2img/fig2_fast_rp.pdf} \\
% % \hspace{-1.5cm}
% \includegraphics[width=5.0cm,height=3.0cm]{figures/ts2img/fig2_slow_lc.pdf} &
% \includegraphics[width=3.5cm,height=3.5cm]{figures/ts2img/fig2_slow_gaf.pdf} &
% \includegraphics[width=3.5cm,height=3.5cm]{figures/ts2img/fig2_slow_mtf.pdf} &
% \includegraphics[width=3.5cm,height=3.5cm]{figures/ts2img/fig2_slow_rp.pdf} \\
% \end{tabular}
% \vspace{-0.0cm}
% \caption{Some representative Light Curves and their corresponding Image Transformations. The \textbf{top row} shows a light curve with a fast rotation period and the \textbf{bottom row} shows a light curve with a slow rotation period along with their respective image transformations } % used as stopping criterion with the 
% \label{fig:ts2img}
% \end{center}
% \end{figure}


% \subsection{Image Transformations}
% \textbf{Add 2. Figure of light curve and image transformation. Maybe make this a panel with different stars that rotate at different speeds?}
